Dark Energy Survey Year 1 Results: Cross-Correlation Redshifts in the DES -- Calibration of the Weak Lensing Source Redshift Distributions

We present the calibration of the Dark Energy Survey Year 1 (DES Y1) weak lensing source galaxy redshift distributions from clustering measurements. By cross-correlating the positions of source galaxies with luminous red galaxies selected by the redMaGiC algorithm we measure the redshift distributions of the source galaxies as placed into different tomographic bins. These measurements constrain any such shifts to an accuracy of $\sim0.02$ and can be computed even when the clustering measurements do not span the full redshift range. The highest-redshift source bin is not constrained by the clustering measurements because of the minimal redshift overlap with the redMaGiC galaxies. We compare our constraints with those obtained from $\texttt{COSMOS}$ 30-band photometry and find that our two very different methods produce consistent constraints.

==> Makefile <==

texfile := main
default: pdf

author:
	mkauthlist -a order.csv -f -j mnras DES-2017-0263_author_list.csv authors.tex
	echo "Now go edit the authors.tex to put the affiliations in affiliations.tex!"

bib: 
	bibtex ${texfile}

pdf: 
	#pdflatex ${texfile}
	latexmk -pdf -g ${texfile}

clean:
	rm -f \
	${texfile}.dvi \
	${texfile}.pdf \
	${texfile}.aux \
	${texfile}.bbl \
	${texfile}.blg \
	${texfile}.toc \
	${texfile}.fls \
	${texfile}.out \
	${texfile}.fdb_latexmk \
	${texfile}.log

